Classical vs Quantum Advice and Proofs under Classically-Accessible Oracle

It is a long-standing open question to construct a classical oracle relative to which BQP/qpoly $\neq$ BQP/poly or QMA $\neq$ QCMA. In this paper, we construct classically-accessible classical oracles relative to which BQP/qpoly $\neq$ BQP/poly and QMA $\neq$ QCMA. Here, classically-accessible classical oracles are oracles that can be accessed only classically even for quantum algorithms. Based on a similar technique, we also show an alternative proof for the separation of QMA and QCMA relative to a distributional quantumly-accessible classical oracle, which was recently shown by Natarajan and Nirkhe.

==> scratch.tex <==
\section{Scratch}

I added here some of the text that did not make the cut, in case they are needed for further work.

\subsection{One-way to Hiding and Yao's box}

For proving \Cref{lem:separation_poly_qpoly_dist}, we prepare the following lemma.
\begin{lemma}\label{lem:query_amplitude}
    Let $G:\bit^n\rightarrow \bit$ be a uniformly random function.  For an unbounded-time algorithm $\A$ that makes $\poly(\secp)$ classical queries to $G$ and a family of $\poly(n)$-bit classical advice $\{z_G\}_{G}$,  suppose that the following holds:
    \begin{align*}
        \Pr_{G,x\la \bit^n}[\A^{G}(z_G,x)=G(x)]> \frac{3}{5}.
    \end{align*}
    For each $x\in \bit^n$, we define the average query magnitude $\delta_x$ on $x$ to be the probability that a measurement of a randomly chosen query by $\A^{G}(z_G,x)$ to $G$ results in $x$ where $G$ is uniformly random. 
    Then for a $1/\poly(n)$-fraction of $x\in \bit^n$, $\delta_x=1/\poly(n)$. 
\end{lemma}
\begin{proof}
    For each $x\in\bit^n$, we can define $G_x$ as following: $G_x(x)=0$, and $G_x(x')=G(x')$ for $x'\neq x$. Assume that $\A$ makes $Q$ queries, we can apply \Cref{lem:o2h} to each $x$, obtaining that 
    \begin{align*}
        |\Pr_{G}[\A^{G}(z_G,x)=G(x)]-
        \Pr_{G}[\A^{G_x}(z_G,x)=G(x)]|\le 2Q \sqrt{\delta_x}.
    \end{align*}
    %\angelos{I think above the probability should be over $x$ too, since we set $S$ from Lemma 2.1 to be $\{x\}$ and we want $S$ to be random? Then the RHS would be $2Q\sqrt{\mathbb{E}[\delta_x]}$? - Resolved, thank you for clarifying!}\takashi{It's a little bit confusing, but "random" in the statement of Lemma 2.1 doesn't mean uniformly random.     As stated in the lemma, we can allow an arbitrary distribution. In particular, it's fine to fix $S$ to be $\{x\}$ for a particular $x$.     }
    Now we consider the case when we uniform randomly choose $x\la\bit^n$, and require $\A^{G_x}(z_G,x)$ to output $G(x)$. This is exactly Yao's box problem, where the adversary is required to output $G(x)$ without querying $x$. By results from~\cite{FOCS:CGLQ20}, we have the following bound for Yao's box:
    \begin{align*}
        \Pr_{G,x}[\A^{G_x}(z_G,x)=G(x)]\leq \frac{1}{2}+\sqrt[3]{\frac{|z_G|Q}{2^n}}=\frac{1}{2}+\negl(n).
    \end{align*}
    %\angelos{I think $S$ in \cite{FOCS:CGLQ20} corresponds to the length of the advice, so the second term should be $\sqrt[3]{\frac{\poly(n)Q}{2^n}} = \negl(n)$}\takashi{Yes, probably can we write  $\sqrt[3]{\frac{|z_G|Q}{2^n}} = \negl(n)$?}
    Thus we have that 
    \begin{align*}
        \Pr_{G,x}[\A^{G}(z_G,x)=G(x)]- \Pr_{G,x}[\A^{G_x}(z_G,x)=G(x)]\geq \frac{1}{10}-\negl(n),
    \end{align*}
    Therefore, we have
    \begin{align*}
        \Ex_x [2Q \sqrt{\delta_x}]\geq \Ex_x [|\Pr_{G}[\A^{G}(z_G,x)=G(x)]&-
        \Pr_{G}[\A^{G_x}(z_G,x)=G(x)]|]\geq \frac{1}{10}-\negl(n)\\
        \Ex_x\sqrt{\delta_x}&\geq\frac{1}{\poly(\secp)}
    \end{align*}
    \angelos{Informal argument:} Say $\mathbb{E}_x[\sqrt{\delta_x}] \geq \frac{1}{q(\secp)}$, where $q$ is a polynomial.
    
    Let $p$ be the probability that a random $x$ satisfies $\delta_x \geq \frac{1}{4q^2(\secp)} \iff \sqrt{\delta_x} \geq \frac{1}{2q(\secp)}$. Then
    $$p + (1 - p)\cdot \frac{1}{2q(\secp)} \geq \mathbb{E}_x[\sqrt{\delta_x}] \geq \frac{1}{q(\secp)}$$
    $$\implies p + \frac{1}{2q(\secp)} \geq \frac{1}{q(\secp)}$$
    Thus for at least an inverse polynomial $\frac{1}{2q(\secp)}$ fraction of $x \in \{0, 1\}^n$, $\delta_x \geq \frac{1}{4q^2(\secp)} = \frac{1}{\poly(n)}$.
    %\xingjian{It seems we can obtain one side of $\Omega(1)$ in the claim?}\takashi{I think both should be $1/\poly$. It may be possible that $\delta_x=1/\poly$ for all $x$. On the other extreme, it may be possible that $\delta_x=1$ for $1/\poly$-fraction of $x$ and $\delta_x=0$ for the rest of $x$.Sorry, I'm a little bit confused. I'll think about it for a while. $1/\poly$ for both would be fine. It would be great if you can write it down. }    \angelos{Okay, let me see what I can do!}\xingjian{I think Takashi is correct, we can only obtain both $1/\poly$.}
\end{proof}

==> zzz_advice_quantum_access.tex <==
% This is a backup for the old manuscript on the separation relative to a quantumly-accessible classical oracle 
\section{Oracle Separation between $\BQP/\poly$ and $\BQP/\qpoly$}\label{sec:advice} 
 We prove the following theorem.
\begin{theorem}\label{thm:separation_poly_qpoly}
There is a classical oracle $\ora$ relative to which $\BQP/\poly\neq \BQP/\qpoly$.
\end{theorem} 
\takashi{By the way, we are actually showing a stronger statement that there is an oracle relative to which $\BQP/\qpoly\cap \NP \cap \coNP\not\subseteq \BQP/\poly$ as the classical solution to the YZ problem can be used as a classical witness for both yes and no. We may want to make it explicit.
Making it even stronger (but less intuitive), we are actually showing an oracle relative to which $\mathsf{YQP}^*\cap \NP \cap \coNP \not\subseteq \BQP/\poly$ where $\mathsf{YQP}^*$ is the class of problems that can be decided by a $\BQP$ machine with \emph{untrusted} quantum advice where the validity of the advice can be tested obliviously on the input. (A related class $\mathsf{YQP}$ was first defined in \cite{Aaronson07} but the definition is revised by \cite{SICOMP:AarDru14} due to a subtle technical issue. Based on the revised definition of $\mathsf{YQP}$, \cite{SICOMP:AarDru14} defined its subclass $\mathsf{YQP}^*$.)
Since $\mathsf{YQP}^*\subseteq \BQP/\qpoly$ for an obvious reason (indeed, \cite{SICOMP:AarDru14} proved $\mathsf{YQP}^*/\poly= \BQP/\qpoly$), the separation is stronger.
}

\takashi{I found that a separation between $\BQP/\poly$ and $\BQP/\qpoly$ relative to a classically-accessible classical oracle seems to imply $\mathsf{FBQP}/\poly\neq \mathsf{FBQP}/\qpoly$ \emph{unconditionally}. (Mathematically speaking, \cite{ABK23} already proved $\mathsf{FBQP}/\poly\neq \mathsf{FBQP}/\qpoly$ unconditonally, so the above statement logically says nothing.
But what I mean is there is a "natural" conversion from  a separation between $\BQP/\poly$ and $\BQP/\qpoly$ relative to a classically-accessible classical oracle into an unconditional separation between $\mathsf{FBQP}/\poly$ and $\mathsf{FBQP}/\qpoly$.) I note that I come up with this observation after reading \cite{ABK23}, so we cannot claim that this is concurrent to theirs.
}

As observed in \cite{EC:Liu23},
\Cref{thm:YZLiu_separation_Ver} (or its weaker version in \cite{EC:Liu23}) already exhibits a separation between the powers of classical and quantum advice in a contrived setting where the algorithm is not allowed to make any online query to $H$ at all. Our idea is to ``hide" $H$ in an outer oracle $\ora$ from which almost no information of $H$ is accessible to $\BQP/\poly$ machines so that we can reduce the problem to the no online query setting.

The main technical lemma needed for proving \Cref{thm:separation_poly_qpoly} is the following.
\begin{lemma}\label{lem:separation_poly_qpoly_dist}
    There are a family of distributions $\{\dist_n\}_{n\in \mathbb{N}}$, where $\dist_n$ is supported on tuples $(G,\ora)$ of functions $G:\bit^n\rightarrow \bit$ and $\ora: \bit^{p(n)}\rightarrow \bit^{q(n)}$ for some polynomials $p$ and $q$, 
    satisfying the following:
    \begin{description}
  \item[Easiness with Quantum Advice]
    There is a QPT algorithm $\A$ with classical access to $\ora$ and a family of $\poly(n)$-qubit quantum advice $\{\rho_\ora\}_{\ora}$
    such that  
    \begin{align*}
        \Pr_{(G,\ora)\la \dist_n}[
    \forall x\in \bit^n~
    \Pr[\A^{\ora}(\rho_\ora,x)=G(x)]\ge 1-\negl(n)
    ]\ge  1-\negl(n).
    \end{align*}
    \item[Hardness with Classical Advice] 
     For any unbounded-time algorithm $\A$ that makes $\poly(\secp)$ classical queries to $\ora$ and a family of $\poly(n)$-bit classical advice $\{z_\ora\}_{\ora}$,  
     \begin{align*}
        \Pr_{(G,\ora)\la \dist_n,x\la \bit^n}[
    \A^{\ora}(z_\ora,x)=G(x) 
    ]
    \le \frac{3}{5}
    \end{align*}
for all sufficiently large $n$.
\end{description}
\takashi{$3/5$ could be any constant between $1/2$ and $2/3$.}
\end{lemma}

\begin{proof}[Proof of \Cref{thm:separation_poly_qpoly}]
\takashi{This is just a sketch, and we need to polish it.}
    \Cref{thm:separation_poly_qpoly} easily follows from \Cref{lem:separation_poly_qpoly_dist} by a standard diagonalization argument. A little bit more precisely, it works as follows.
    Suppose that we generate $(G_n,\ora_n)\la \dist_n$ and define a language $\calL:=\bigsqcup_{n\in \mathbb{N}}G_n^{-1}(1)$ and an oracle $\ora$ that returns $\ora_{|x|}(x)$ on a query $x\in \bit^*$.  
    We claim that $\calL\in \BQP^{\ora}/\qpoly$ and $\calL\notin \BQP^{\ora}/\poly$ with probability $1$. 
    
    To see $\calL\in \BQP^{\ora}/\qpoly$, the first condition of \Cref{lem:separation_poly_qpoly_dist} implies that there is 
    a
    $\BQP^{\ora}/\qpoly$ machine $M$ that decides $\calL$ on all $x$ of length $n$  with probability at least $1-\frac{1}{n^2}$ for all sufficiently large $n$. 
    For any sufficiently large $N$, 
    by the union bound, 
    the probability that  $M$ fails to decide $\calL$ on any $x$ of length $n\ge N$ is at most $\sum_{n=N}^{\infty}\frac{1}{n^2}$.    Note that   $\lim_{N\rightarrow \infty}\sum_{n=N}^{\infty}\frac{1}{n^2}=0$ because $\sum_{n=1}^{\infty}\frac{1}{n^2}=\pi^2/6$, which is in particular finite.  
    Therefore, the probability that there is $N$ such that  $M$ succeeds in deciding $\calL$ on all $x$ such that $|x|\ge N$ is $1$.
    By augmenting $M$ to decide $\calL$ by brute-force when the instance is length is smaller than $N$, we can conclude that there is a  $\BQP^{\ora}/\qpoly$ machine that decides $\calL$ on all $x\in \bit^*$ with probability $1$ over the random choice of $(G_n,\ora_n)$ for $n\in \mathbb{N}$. 

    To see $\calL\notin \BQP^{\ora}/\poly$,  the second condition of \Cref{lem:separation_poly_qpoly_dist} implies that
    for any $\BQP$ machine $M$ with quantum oracle access to $\ora$ and a polynomial-size classical advice that depends on $\ora$, the probability that  it succeeds in deciding $\calL$ on all $n$-bit $x$ is at most $9/10$
    for all sufficiently large $n$. 
    Since the event that $M$ succeeds in deciding  $\calL$ on all $n$-bit $x$ is independent for each $n$, 
    the probability that $M$ succeeds in deciding $\calL$ on all $x\in \bit^*$ is $0$. 
    Since there are only countably many $\BQP$ machines, the probability that there is $M$ that succeeds in deciding $\calL$ on all $x\in \bit^*$ is $0$.  
\end{proof}

For proving \Cref{lem:separation_poly_qpoly_dist}, we prepare the following lemma.
\begin{lemma}\label{lem:query_amplitude}
    Let $G:\bit^n\rightarrow \bit$ be a uniformly random function.  For an unbounded-time algorithm $\A$ that makes $\poly(\secp)$ classical queries to $G$ and a family of $\poly(n)$-bit classical advice $\{z_G\}_{G}$,  suppose that the following holds:
    \begin{align*}
        \Pr_{G,x\la \bit^n}[\A^{G}(z_G,x)=G(x)]> \frac{3}{5}.
    \end{align*}
    For each $x\in \bit^n$, we define the average query probability $\delta_x$ on $x$ to be the probability that a randomly chosen query by $\A^{G}(z_G,x)$ to $G$ is equal to $x$ where $G$ is uniformly random. 
    Then for a $1/\poly(n)$-fraction of $x\in \bit^n$, $\delta_x=1/\poly(n)$. 
\end{lemma}
\begin{proof}
    For each $x\in\bit^n$, we can define $G_x$ as following $G_x(x')=\begin{cases}0 & \text{if}~x' = x \\ G(x') & \text{if}~x' \neq x \end{cases}$. Since $\A$ only makes classical queries to $G$, the only way for it to distinguish $G$ from $G_x$ is to query the oracle at $x$. Assume that $\A$ makes $Q$ queries, then for each $x$, we obtain that 
    \begin{align*}
        |\Pr_{G}[\A^{G}(z_G,x)=G(x)]-
        \Pr_{G}[\A^{G_x}(z_G,x)=G(x)]|\le Q \delta_x.
    \end{align*}
    %\angelos{I think above the probability should be over $x$ too, since we set $S$ from Lemma 2.1 to be $\{x\}$ and we want $S$ to be random? Then the RHS would be $2Q\sqrt{\mathbb{E}[\delta_x]}$? - Resolved, thank you for clarifying!}\takashi{It's a little bit confusing, but "random" in the statement of Lemma 2.1 doesn't mean uniformly random.     As stated in the lemma, we can allow an arbitrary distribution. In particular, it's fine to fix $S$ to be $\{x\}$ for a particular $x$.     }
    Now we consider the case when we uniform randomly choose $x\la\bit^n$, and require $\A^{G_x}(z_G,x)$ to output $G(x)$. This is exactly Yao's box problem, where the adversary is required to output $G(x)$ without querying $x$. By results from~\cite{C:DeTreTul10} \angelos{As Takashi said, they don't explicitly prove it, but e.g. Lemma 8.4 seems related}, we have the following bound for Yao's box with classical queries and classical advice:
    \begin{align*}
        \Pr_{G,x}[\A^{G_x}(z_G,x)=G(x)]\leq \frac{1}{2}+\sqrt{\frac{|z_G|Q}{2^n}}=\frac{1}{2}+\negl(n).
    \end{align*}
    %\angelos{I think $S$ in \cite{FOCS:CGLQ20} corresponds to the length of the advice, so the second term should be $\sqrt[3]{\frac{\poly(n)Q}{2^n}} = \negl(n)$}\takashi{Yes, probably can we write  $\sqrt[3]{\frac{|z_G|Q}{2^n}} = \negl(n)$?}
    Thus we have that 
    \begin{align*}
        \Pr_{G,x}[\A^{G}(z_G,x)=G(x)]- \Pr_{G,x}[\A^{G_x}(z_G,x)=G(x)]\geq \frac{1}{10}-\negl(n),
    \end{align*}
    Therefore, we have
    \begin{align*}
        \Ex_x [Q \delta_x]\geq \Ex_x [|\Pr_{G}[\A^{G}(z_G,x)=G(x)]&-
        \Pr_{G}[\A^{G_x}(z_G,x)=G(x)]|]\geq \frac{1}{10}-\negl(n)\\
        \implies \Ex_x[\delta_x]&\geq\frac{1}{\poly(\lambda)}
    \end{align*}
    Choose $q(\lambda)$ to be a polynomial such that $\mathbb{E}_x[\delta_x] \geq \frac{1}{q(\lambda)}$.
    
    Let $p$ be the probability that a random $x$ satisfies $\delta_x \geq \frac{1}{2q(\lambda)}$. Then
    $$p + (1 - p)\cdot \frac{1}{2q(\lambda)} \geq \mathbb{E}_x[\delta_x] \geq \frac{1}{q(\lambda)}$$
    $$\implies p + \frac{1}{2q(\lambda)} \geq \frac{1}{q(\lambda)}$$
    Thus for at least an inverse polynomial $\frac{1}{2q(\lambda)}$ fraction of $x \in \{0, 1\}^n$, $\delta_x \geq \frac{1}{2q(\lambda)} = \frac{1}{\poly(n)}$.
    %\xingjian{It seems we can obtain one side of $\Omega(1)$ in the claim?}\takashi{I think both should be $1/\poly$. It may be possible that $\delta_x=1/\poly$ for all $x$. On the other extreme, it may be possible that $\delta_x=1$ for $1/\poly$-fraction of $x$ and $\delta_x=0$ for the rest of $x$.Sorry, I'm a little bit confused. I'll think about it for a while. $1/\poly$ for both would be fine. It would be great if you can write it down. }    \angelos{Okay, let me see what I can do!}\xingjian{I think Takashi is correct, we can only obtain both $1/\poly$.}
\end{proof}

Then we prove \Cref{lem:separation_poly_qpoly_dist}.
\begin{proof}[Proof of \Cref{lem:separation_poly_qpoly_dist}]
We define $\dist_n$ to be the distribution that samples $G$ and $\ora$  as follows:
\begin{description}
    \item[$\dist_n$:] %For each $x\in \bit^n$, it puts $x$ into $S$ with probability $1/2$ independently. 
    Let  $C\subseteq \Sigma^n$ be the code in \Cref{cor:YZLiu_separation_classical_query_amp}. 
  It samples random functions $G:\bit^n\rightarrow \bit$ and $H^{(j)}:\bit^{\log n}\times \Sigma \rightarrow \bit$ for $j\in [n]$
  and defines $\ora$ as follows:
  $\ora$ takes $x\in \bit^n$ and $(\vv^{(1)},...,\vv^{(n)})\in C^n$ as input, and outputs $G(x)$ if 
 there is $j\in [n]$ such that
 $f_C^{H^{(j)}}(\vv^{(j)})=x$ and outputs $0$ otherwise.\footnote{Note that $x$ here plays the role of $r$ in \Cref{cor:YZLiu_separation_classical_query_amp}.} 
\end{description} 
First, we show the easiness with quantum advice. 
Let $(\A',\{\rho'_H\}_H)$ the tuple of an algorithm and family of quantum advice in the first condition of \Cref{cor:YZLiu_separation_classical_query_amp}. 
We construct $(\A,\{\rho_\ora\}_{\ora})$ that satisfies the first condition of \Cref{lem:separation_poly_qpoly_dist} as follows:
\begin{description}
    \item[$\rho_\ora$:] 
    We describe a randomized procedure to set $\rho_\ora$ given an oracle $\ora$. 
    This should be understood as setting $\rho_\ora$ to be the mixed state corresponding to the output of the procedure.  
    Sample $(G,H)$ from the conditional distribution of $\dist_n$ conditioned on the given $\ora$. Note that then the joint distribution of $(G,H,\ora)$ is identical to the real one. Then $\rho_\ora$ is set to be $\rho_H$.
    More precisely, $\rho_\ora$ should be defined to be the mixed state that correspond to the output of the above randomized procedure. 
    \item[$\A^\ora(\rho_\ora,x)$:] 
    It runs $\vv\la \A'(\rho_\ora,x)$, queries $(x,\vv)$ to $\ora$, and outputs whatever $\ora$ returns.  
\end{description}
Then the first condition of  \Cref{lem:separation_poly_qpoly_dist} directly follows from the first condition of \Cref{cor:YZLiu_separation_classical_query_amp}. 

Next, we show the hardness with classical advice.
Suppose that there is $(\A,\{z_\ora\}_{\ora})$ that breaks it. Then we have 
    \begin{align*}
        \Pr_{\substack{(G,\ora)\la \dist_n \\x\la \bit^n}}[
    \A^{\ora}(z_\ora,x)=G(x) 
    ]
    > \frac{3}{5}
    \end{align*}
    for infinitely many $n\in \mathbb{N}$.
Note that the only way for $\A$ to learn $G(x)$ is to query $(x,\vv)$ such that $f_C^H(\vv)=x$ to
$\ora$. Thus, by a direct reduction to \Cref{lem:query_amplitude}, 
for an $\Omega(1/\poly(\lambda))$-fraction of $x\in \bit^n$, 
if we consider a randomly chosen query by $\A^\ora(z_\ora,x)$ for a randomly chosen $\ora$ according to $\dist_n$, then with probability $\Omega(1/\poly(\lambda))$, the query is $(x,(\vv^{(1)},...,\vv^{(n)}))$ such that there is $j\in [n]$ such that $f_C^{H^{(j)}}(\vv^{(j)})=x$.  
Note that $\ora$ can be simulated by $G$ and the verification oracle $\Ver_{C}^H=(\Ver_{C}^{H^{(1)}},...,\Ver_{C}^{H^{(n)}})$, and a direct access to $H=(H^{(1)},...,H^{(n)})$ is not needed for the simulation. 
Thus, the above directly gives an algorithm that violates the hardness with classical advice and verification oracle (the second item of \Cref{cor:YZLiu_separation_classical_query_amp}). 
Specifically, we construct $(\A',\{z'_H\}_H)$ that violates the second item of \Cref{cor:YZLiu_separation_classical_query_amp} as follows:
\begin{description}
    \item[$z'_H$:] Randomly choose $G$ and construct $\ora$ from $(G,H)$. Set $z'_H:=(G,z_\ora)$. \takashi{I'm writing it as if $z'_H$ is randomized while that should be deterministic. But this doesn't matter; we can derandomize it by choosing the best one. We may need to add some remark (or change the way of the explanation).} 
    \item[${\A'}^{\Ver_{C}^H}((G,z_\ora),x)$:] 
    It runs $\A^{\ora}(z,x)$ where it chooses a random query by $\A$ to get $(x',(\vv^{(1)},...,\vv^{(n)}))$, and outputs $(\vv^{(1)},...,\vv^{(n)}))$. 
    Note that ${\A'}^{\Ver_{C}^H}$ can simulate $\A^\ora$ because classical access to $\ora$ can be simulated by using classical access to $G$ and its own oracle $\Ver_{C}^H$ as explained above.
\end{description}
For the output $(\vv^{(1)},...,\vv^{(n)}))$ of $\A'$, there is $j\in [n]$ such that $f_C^{H^{(j)}}(\vv^{(j)})=x$ 
with probability $1/\poly(\secp)$ over the random choice of $H$ and $x\la \bit^n$ (for infinitely many $n\in\mathbb{N}$). This contradicts \Cref{cor:YZLiu_separation_classical_query_amp}. 
\end{proof}


\iffalse
\takashi{The following is my thoughts on how to remove the verification oracle.}
\takashi{This turns out to not work.}
\begin{lemma}
    Let $G:\bit^n\rightarrow \bit$ and $G':\bit^n\rightarrow \bit$ be uniformly random functions. 
    For any family of $\poly(n)$-bit classical advice $\{z_{G,G'}\}_{G,G'}$, there is a family $\{S_{G,G'}\}_{G,G'}$ of subsets of $\bit^n$ of size $\poly(n)$ such that for any unbounded-time algorithm $\A$ and any 
    \begin{align*}
        |\Pr_{G,G'}[\A(z_{G,G'},\{G(x)\}_{x\in \bit^n\setminus S_{G,G'}})=1]-\Pr_{G,G'}[\A(z_{G,G'},\{G'(x)\}_{x\in \bit^n\setminus S_{G,G'}}))=1]| \le \negl(n)
    \end{align*}
\end{lemma}
\takashi{Does this lemma make sense? If we can prove this lemma, we may not need to prove the hardness against adversaries with the verification oracle based on idea described in my email.}
\angelos{From what I understand, $S_{G, G'}$ are the indices that you fix in this classical-BF-QROM. In your email, you suggest the following: ``But what if we modify the response of $\ora$ in the invalid case to $G'(x)$ for another random function $G'$''? I agree that now each query to $O$ will look random, but the values of more than one queries may leak some information about $H$? For example, $O(x, v) = G'(x)$ for almost every codeword $v$, whereas $O(x, v) = G(x)$ for only a small fraction of codewords $v$. }
\takashi{Yes, you are right, and my idea doesn't work. Basically, returning $G'(x)$ is no better than returning $0$ because you can learn $G'(x)$ by querying $(x,\vv)$ for random $\vv$ which is invalid whp.}
\fi
